Large Language Model-Guided Prediction Toward Quantum Materials Synthesis

The synthesis of inorganic crystalline materials is essential for modern technology, especially in quantum materials development. However, designing efficient synthesis workflows remains a significant challenge due to the precise experimental conditions and extensive trial and error. Here, we present a framework using large language models (LLMs) to predict synthesis pathways for inorganic materials, including quantum materials. Our framework contains three models: LHS2RHS, predicting products from reactants; RHS2LHS, predicting reactants from products; and TGT2CEQ, generating full chemical equations for target compounds. Fine-tuned on a text-mined synthesis database, our model raises accuracy from under 40% with pretrained models, to under 80% using conventional fine-tuning, and further to around 90% with our proposed generalized Tanimoto similarity, while maintaining robust to additional synthesis steps. Our model further demonstrates comparable performance across materials with varying degrees of quantumness quantified using quantum weight, indicating that LLMs offer a powerful tool to predict balanced chemical equations for quantum materials discovery.

==> archive/introduction_240918.tex <==
\section{Introduction}
As scientific research advances, it naturally leads us to tackle increasingly challenging problems. Over the past century, we have observed the trend of increasing our classical computational power to meet the demand for solving such complex problems. However, we currently find ourselves on the brink of computational intractability with existing methods, posing a significant obstacle to further progress.

One avenue is through materials informatics, which harnesses computational techniques, such as machine learning and quantum simulations, to expedite the discovery of materials with specific properties. By training models on large databases of material properties, researchers can identify novel materials candidates with the potential to revolutionize computation. Exploring unconventional materials, such as topological insulators or quantum materials, may offer new ways to overcome computational bottlenecks.

Crystals are a class of inorganic materials, distinguished by their regular, repeating pattern of atoms or molecules arranged in a three-dimensional lattice structure. They stand apart from molecules, which consist of specific atoms bonded together but lack the same ordered arrangement. They can be categorized into polycrystals, composed of multiple crystalline domains with varying orientations, and single crystals, which feature a continuous lattice throughout the entire sample. In semiconductors, the ordered lattice structure allows for controlled manipulation of electron flow, crucial for devices like transistors and diodes. In insulators, the lattice structure creates a wide band gap, making them excellent materials for electrical insulation and dielectric applications.

Crystal synthesis methods involve combining solutes with different compounds through techniques often involving heating to dissolve the solute in the compound, followed by cooling to precipitate crystalline structures. Synthesizing materials with properties optimized for computation presents a significant challenge; the conventional dependence on human intuition to navigate the uncharted state space of synthesis parameters is marked by inefficiencies, becoming more evident as the duration for crystal growth extends from weeks to years. This limitation underscores the need for informed crystal growth, aimed at predicting promising synthesis parameters to reduce bottlenecks and avoid redundant crystal growth.

Understanding the underlying chemical equations is an important part of this problem. By representing the underlying chemical transformations, these equations guide the selection of optimal synthesis conditions and initial substrates to achieve specific properties in resultant materials.

However, predicting chemical reactions is a challenging task. Combinatorial chemistry and materials science have shown that the space of inorganic materials grows exponentially with the number of components. This growth makes navigating and identifying viable materials challenging due to the vast number of possible combinations and constraints such as chemical stability, mechanical properties, and cost-effectiveness. For example, it is estimated that there are around $\sim$10$\textsuperscript{13}$ stable compounds consisting of five different elements\cite{Davies2016-qx}. Previous work on computational materials discovery explores the performance of Graph Neural Networks (GNNs) on data from the Materials Project\cite{kononova2019text,jain2013commentary, wang2022dataset} to predict inter-atomic energy potentials of generated materials with NequIP\cite{EquivarianceNequIP, ScalingDLforMatDisc}. By training on the atomic structures which are governed by Euclidean symmetry in three dimensions, intra-molecular positional relationships can be exploited to reduce the parameter space, thereby improving the model's efficiency and accuracy in predicting material properties. MatterGen \cite{zeni2024mattergen}, a generative model from Microsoft involves a diffusion-based approach to explore the same space of novel materials.

While chemical compounds exhibit geometric characteristics seemingly separate from sequential language data, transformers\cite{Vaswani} can bridge this gap by encoding and processing the spatial arrangements and relationships within chemical structures as sequences. This ability allows them to apply the same techniques used for natural language processing to the domain of chemistry. By treating chemical notation and synthesis procedures as a form of language, transformers can capture underlying patterns, effectively predicting reactions and operations based on textual representations of molecular transformations. The contemporary approach for computational materials discovery, pioneered by NequIP and MatterGen, is to train on compounds' spatial relationships, because it eliminates the semantic translation errors that can occur when converting raw chemical representations into human language descriptions. Therefore, abstraction and avoiding bias towards human language expressions are crucial when using transformers to predict chemical transformations, as this ensures that the model accurately captures the intrinsic properties and relationships within the chemical data without being influenced by the nuances and potential inaccuracies of human linguistic interpretation.

We approach the problem of materials discovery from a practical viewpoint, aiming to develop models that predict the full chemical equation (and occasionally synthesis operations) from partial inputs; these can assist in experimentation when a researcher has incomplete information.

We have outlined machine learning models that hold promise in facilitating materials discovery, but we have yet to establish the data necessary for training these models to learn effectively. The vast majority of scientific data is written in scientific journals, and chemical equations lack the nuance and flexibility of written language, so we need to efficiently extract data specific to our project from these journals. Text mining techniques offer a solution to this challenge by enabling the parsing of relevant information from these unstructured texts. Therefore, we can funnel this abundance of unstructured information into ordered data for training models on inorganic crystal synthesis processes.

In this work, we explore the application of LLMs for learning chemical equations involved in crystal synthesis. By fine-tuning the GPT2 model on text-mined data comprising crystal synthesis procedures and chemical reactions, we aim to predict chemical equations with synthesis operations. Our results demonstrate the efficacy of the proposed method in predicting chemical reactions and synthesis operations, for the goal of advancing in materials discovery.


- we should highlight that, we could run the prediction even with the small model go GPT like distilGPT2.   \\
- we observed that LLM presents a similar intuition as the human scientists, that predicting reactant (or LHS) is easier than predicting LHS. \\
- Our finee-tuned LLM models are robust against the added text, by fine-tuning the model with added prompts. 



==> archive/method_240917.tex <==
\section{Method}
\subsection*{Overview}

 Figure \ref{fig_overview} shows the set of models--which we denote the LLM module--that predict chemical equations and synthesis operations from known incomplete partitions. 

briefly cover:  \\
- data preparation 
- load pre-trained GPT model from HF \\
- fine-tune the model using the Ceder group's dataset 
-  evaluation of the model. 
- We have three kinds of models: LHS2RHS, RHS2LHS, TGT2CEQ
- Effect of added text (related but not very obviously be related) to the generated text. To present the robustness (todo: to include this into the figure)  
- Here we present many of the abbreviations: left hand side(LHS), right hand side (RHS), target compound (TGT), chemical equation(CEQ), synthesis operation (OPE). 


\begin{figure}[ht!]
\includegraphics[width=\textwidth]{figures/fig_m_tmp.png}
\caption{\textbf{Overview of models for chemical synthesis prediction:}  Prepare data, load a model, fine-tune the model, and evaluate it.
}
\label{fig_overview}
\end{figure}



\subsection*{Data preparation}

-  text-mined database from Ceder group \\
- check the abstract and a bit method section of the original paper. 

Fine-tuning data is obtained from the CEDER dataset of chemical operations, which contains 19488 inorganic synthesis recipes extracted from scientific journals (5798 are registered in the Materials Project database). 

- Define the Ceder database and add a brief explanation. 

- data processing   \\
- data representation   \\
- connect the chemical equation with '$->$' \\
- if we use the synthesis operations (OPE) as the additional prompts, we simplify the synthesis operations in the CEDER dataset to only the operation names, such as 'Mix Mix Heat Dry'. 
- For simplicity and consistency, here we skip the details of the experimental condition, such as the heating temperature, the temperature profile, and the time spent for each operation. 
- the list of operation terms: 'SolutionMix', 'Shape', 'Dry', 'Mix', 'Heat', 'LiquidGrind', 'Quench'
% - As one benchmark, we prepared the dataset with irrational synthesis operations, which randomly arranged the synthesis operations. This dataset was used to verify the robustness of the model against the additional text prompt with no relevance. --> skip!
- we set the separator, which specifies the boundary of the prompt and the answer. 
- prompt and the true text 
- remove the unnecessary text after the chemical equation (split by ';'). 
- train, test split, 9:1



\subsection*{Fine-tuning the model}
- Fine-tune the language model: an introduction. 
- we use the distilGPT2 model as the pre-trained model, which can be accessed from HuggingFace. 
- we used the Huggingface API and transformer library to load the model. 
- we referenced distilbert/distilgpt2 to load the model using the class AutoModelForCausalLM.
- We loaded the tokenizer using the AutoTokenizer class. 
- Data collator (DataCollatorForLanguageModeling).
- We used Trainer to fine-tune the model.
- hyperparameters 
lr=2e-5, 
wdecay=0.01, 
per-device-train-batch-size = 4,  
- cross-validation: 100 epochs, 10-fold cross-validation. We trained the model twice and spent 200 epochs so that the loss function ultimately converges. 
- more explanation about distilGPT2 (difference from GPT2)? check the HF page.  


\subsection*{Text Inference and Evaluation}
. Text generation: introduction.    \\
- We used the fine-tuned model to predict the chemical equation of our target. 

- the chemical equation does need to be the 

- Option for the text generation (e.g., greedy decoding, multinomial sampling, beam-search decoding). We use XXX. 
- parameter: ('num beams':2, 'do sample':True, 'num beam groups':1) 
- other hyperparameters

- Autoregressive text generation model can generate redundant text by repeating the same phrases repeatedly. We can force the generated text to terminate at some specified lengths to avoid too much text. 
- We can guess the lengths of the chemical equation outputs by searching the correlation of the input and output text (e.g. LHS vs RHS). 
- However, this time we want to evaluate the prediction accuracy of the generated text, so we terminate the text by exactly the same  as the ground truth equations. Note that deciding the termination  is valid only when we know the ground-truth equation. 
- SI analyzes the relationship of the text lengths of LHS, RHS, TGT, and CEQ. 

. Evaluation    \\
- why is evaluation critical, and what is the challenges   \\
- evaluation of the predicted text is important in LLM project.     \\
- There exists language evaluation methods such as Levenshtein, cosine similarity, Jaccard, BLEU, ROUGE, ... \\
- the use of the evaluation function varies depending on the purpose, like whether we value the correspondence of single characters or close context even with different writing expressions.   \\
- for our work of chemical equation prediction, we need to model an intuition to see if the generated chemical equation is correct based on chemical knowledge. 
- When the generated text is a chemical equation, we need a unique evaluation method.  
- what is unique about the chemical equation prediction.    \\
- chemical equations are different from the human conversation language in that they are organized with chemical symbols, numerical symbols, and some special symbols.  
- both LHS and RHS are organized with several chemical formulas connected with '+' symbols     \\
- Write (overly) what it means the LLM can learn the chemical equation (we might move this part to the discussion section later..) 
- assuming each compound is stable, LLM can understand the nature of chemical reactions to find the combination of elements that can stay stable. 
- Charge neutrality needs to be balanced.  
- the number of electrons are also an important aspect to find stable compounds (although we do not explicitly present the information in the text data) 
- Overall, LLM need to understand the relation of the periodicity of the elements. 

- when we compare the corresponding chemical symbols. We can accept the permutation of the chemical species.    \\
- for example, we can identify that 'NaCl' and 'ClNa' as the same compounds, thus we should give zero as the penalty of the prediction.     \\
- we can also accept the permutation of the chemical formula within one side of the chemical equation.  \\
- for example, 'HCl + NaOH' and 'NaOH + HCl' should be identified as the same equations.  \\
- On the other hand, when we evaluate the accuracy of full chemical equation prediction, we need to make sure LHS and RHS do not mix with each other. \\
- We split the chemical equation with $->$, and evaluate LHS and RHS separately. We then take the average of LHS and RHS as the accuracy of the total equations.   \\

- We used the Tanimoto similarity\cite{bajusz2015tanimoto, holliday2003analysis, godden2000combinatorial} to evaluate the similarity of the chemical formula. The Tanimoto similarity, an extension of the Jaccard index, is calculated as the ratio of the intersection's size to the union's size of two vectors, which, in our case, are vectorized compounds. 

- Tanimoto similarity can be used to compare the similarity of the two chemical formulas, but we have adapted Tanimoto similarity to evaluate the similarity of the chemical equation in either one side or the full equation.  

- We average the Tanimoto coefficients across the bijective mapping between ground truth compounds and predicted compounds, resulting in naively a “similarity score” as a performance metric. Outputs range from 0 to 1, indicating no relation and identical vectors, respectively. It is also computationally efficient, avoiding high-dimensional distance calculations. \\

- !Write how we vectorize the chemical formula or the generated text as the list of vectors. 
- given either LHS or RHS of the chemical equation, we split it by the symbols '+', which provides a list of chemical formulas. 
- Given a chemical formula, we first convert a chemical formula into a set of elements.
- First we parse the formula to retrieve the element and index data. We search which elements exist within a chemical formula. Chemical symbols are written by either a single capital letter (e.g., H, B, C, O) or one capital and one lowercase (e.g., Ca, Fe, Na). Once we list up the elements in the formula, we then associate the pairs of the chemical elements and the indices by representing them as a dictionary format. For example, formula "Na2CO3" can be decomposed as "{'Na': 2, 'C': 1, 'O': 3}".
- we do this for all of the formulas in two chemical equations: the generated equation $\mathbf{A}$ and the ground truth $\mathbf{B}$. 
- We calculate the similarity matrix ($N_\text{true}$, $N_\text{pred}$): whose (i, j)-element represents the similarity score of i-th formula in ground-truth equation $A_i$ (total $N_\text{true}$ terms) and j-th formula of the predicted equation $B_j$ (total $N_\text{pred}$ terms). 
- for each pair of the chemical formula ($A_i$, $B_j$), we list the chemical species that commonly exist in both equations. We sum up the product of the index for all common elements. They are the dot products of the two vector-embedded formulas for each of the common elements ($A_i\cdot B_j$) (can we write it with equation?). 

- sum square: Get the square lengths and sum over the two equations. $\|A_i\|^2 + \|B_j\|^2 $. 

- Tanimoto similarity to evaluate the similarity between the two formulas, A and B. 
- Note this method can consider the permutation of chemical elements within a formula. 

%%%%%%%%%%%%%

!! Begin here

The Tanimoto similarity is widely used to evaluate the similarity between two chemical compositions based on their elemental compositions. Given two chemical formulas, the similarity can be computed by treating each formula as a vector in the space of elemental counts. Let us define the two chemical formulas $comp_1$ and $comp_2$. These formulas can be represented as vectors $\mathbf{v}_1$ and $\mathbf{v}_2$, where each component corresponds to the count of a particular element in the composition.

First, we represent the elemental composition of a formula by a vector of element counts. For each chemical formula, we extract the elements and their respective counts and represent the formula as a vector:

\[
\mathbf{v}_1 = \{ \text{element}_1: c_{11}, \text{element}_2: c_{12}, \dots \}
\]
\[
\mathbf{v}_2 = \{ \text{element}_1: c_{21}, \text{element}_2: c_{22}, \dots \}
\]

where $c_{ij}$ is the count of element $i$ in composition $j$. The similarity is calculated by first determining the common elements between the two vectors, $\mathbf{v}_1$ and $\mathbf{v}_2$, denoted by the set of common elements $E_{\text{common}}$. The dot product between these two vectors is calculated as:

\[
\text{dot\_product} = \sum_{\text{element} \in E_{\text{common}}} c_{1,\text{element}} \times c_{2,\text{element}}
\]

Next, we compute the sum of squares of the counts in both vectors:

\[
\text{sum\_squares}_1 = \sum_{\text{element} \in \mathbf{v}_1} c_{1,\text{element}}^2
\]
\[
\text{sum\_squares}_2 = \sum_{\text{element} \in \mathbf{v}_2} c_{2,\text{element}}^2
\]

Finally, the Tanimoto similarity $T(\mathbf{v}_1, \mathbf{v}_2)$ is defined as:

\[
T(\mathbf{v}_1, \mathbf{v}_2) = \frac{\text{dot\_product}}{\text{sum\_squares}_1 + \text{sum\_squares}_2 - \text{dot\_product}}
\]

This formula ensures that the similarity ranges from 0 (no similarity) to 1 (identical compositions). If the two compositions share no common elements, the similarity is zero. Otherwise, the value reflects the proportional overlap in their elemental compositions.

The Python function \texttt{tanimoto\_similarity\_elemental} implements this approach by first converting each chemical formula into a vector of element counts, computing the necessary dot product and sum of squares, and finally applying the Tanimoto similarity formula to return the similarity score.

!!


In the context of chemical equations, evaluating the similarity between two equations requires splitting them into their constituent chemical formulas, specifically the reactants and products. For each equation, we first parse the reactants and products by splitting the equation at the reaction arrow (commonly represented as "$\rightarrow$"). The formulas in each part are further broken down into individual components (i.e., chemical formulas), which are used for comparison.

Let us define two chemical equations, $eq_1$ and $eq_2$, where each equation contains a set of reactants and products. Denote the set of reactants and products for each equation as $\mathbf{R}_1$, $\mathbf{P}_1$, $\mathbf{R}_2$, and $\mathbf{P}_2$. To compare these equations, we first split them into their respective reactants and products:

\[
eq_1: \mathbf{R}_1 \rightarrow \mathbf{P}_1
\]
\[
eq_2: \mathbf{R}_2 \rightarrow \mathbf{P}_2
\]

Once the equations are split into reactants and products, we compare each component using the Tanimoto similarity. For each pair of formulas in the reactant sets $\mathbf{R}_1$ and $\mathbf{R}_2$, we compute their similarity based on their elemental compositions. The Tanimoto similarity between two formulas, $\mathbf{v}_1$ and $\mathbf{v}_2$, is defined as:

\[
T(\mathbf{v}_1, \mathbf{v}_2) = \frac{\text{dot\_product}}{\text{sum\_squares}_1 + \text{sum\_squares}_2 - \text{dot\_product}}
\]

where $\text{dot\_product}$ represents the sum of the product of element counts shared by both formulas, and $\text{sum\_squares}_1$ and $\text{sum\_squares}_2$ are the sums of the squares of the element counts for each formula. The same process is applied to compare the product sets, $\mathbf{P}_1$ and $\mathbf{P}_2$.

To account for the entire equation, the overall similarity is computed as the average of the reactants and products similarities:

\[
\text{similarity}_{\text{overall}} = \frac{T(\mathbf{R}_1, \mathbf{R}_2) + T(\mathbf{P}_1, \mathbf{P}_2)}{2}
\]

In addition to the Tanimoto similarity, the Jaccard similarity is employed as a benchmarking metric. The Jaccard similarity measures the similarity between two sets by comparing their intersection and union. For two sets of formulas (e.g., reactants or products), the Jaccard similarity is given by:

\[
J(A, B) = \frac{|A \cap B|}{|A \cup B|}
\]

where $A$ and $B$ represent the sets of elements in the respective formulas. The Jaccard similarity helps to quantify the structural similarity of the chemical equations based on the overlap of their components.

Thus, by combining both Tanimoto and Jaccard similarities, we can evaluate the similarity between two chemical equations comprehensively, taking into account both the elemental composition and the overall structural correspondence of the reactants and products.



!! End here

%%%%%%%%%%%%%%

 
 \begin{equation}
Tanimoto(A_i, B_j) = \frac{A_i\cdot B_j}{\|A_i\|^2 + \|B_j\|^2 - A_i\cdot B_j}
\label{eq_tanimoto}
\end{equation}

- linear sum assignment (from scipy) to find the matching pairs with the highest similarity score from the two equations, 


- the more common formulas, the higher the overall similarity score becomes.    \\

- This takes the permutation of the chemical formulas in the equation.     \\


- If we evaluate the full chemical equation (TGT2CEQ and TGTOPE2CEQ), we split the chemical equation with $->$, and evaluate LHS and RHS separately. We then take the average of LHS and RHS, as the accuracy of the total equations.   \\


This is similar to Jaccard's similarity. One distinct point of our Tanimoto similarity score is that it accepts the permutation of the atoms within the formula, as well as the naive evaluation of chemical formula. While Jaccard similarity require each of the predicted formula to be exactly the same as the ground-truth, our Tanimoto similarity score take the similarity, even if the two formula are not exactly the same. 


- As the benchmarking evaluation function, we apply Jaccard similarity.   \\
- Jaccards score is used for vectors that take discrete values, most often for binary values (1 or 0). Tanimoto score is used for vectors that can take on continuous values
- brief explanation of Jaccard similarity 
- Equation \ref{eq_jaccard} for Jaccard similarity \\

 \begin{equation}
Jaccard(\mathbf{A}, \mathbf{B}) = \frac{\|\mathbf{A} \cap \mathbf{B}\|}{\|\mathbf{A} \cup \mathbf{A}\|}
\label{eq_jaccard}
\end{equation}

- Here, $\mathbf{A}$ and $\mathbf{B}$ are the set of text components, which is given by splitting the given chemical equation with space. $\|\mathbf{A} \cap \mathbf{B}\|$ count the number of text components that exactly matched between $\mathbf{A}$ and $\mathbf{B}$. $\|\mathbf{A} \cup \mathbf{B}\|$ counts the union of the text components in $\mathbf{A}$ and $\mathbf{B}$. 
- JAC gives an accuracy score only if any of the chemical equations exactly corresponds.    \\
- The normal JAC similarity does not separate LHS and RHS. It evaluate them altogether. Therefore, even if one LHS term shows up on RHS, we can regard it as the correct answer.    \\

- I may consider a better (or simpler) way to evaluate the chemical equations.  \\


\begin{figure}[ht!]
\begin{center}
\includegraphics[width=\textwidth]{figures/fig_m_similaritymethod.png}
\caption{Similarity score calculation method}
\label{fig_similaritymethod}
\end{center}
\end{figure}


 




==> archive/method_240918.tex <==
\section{Method}
\subsection*{Overview}

 Figure \ref{fig_overview} shows the set of models--which we denote the LLM module--that predict chemical equations and synthesis operations from known incomplete partitions. 

briefly cover in the figure, caption, and manuscript:  \\
- data preparation: text-mined synthesis method database.   \\ 
- load pre-trained GPT model from HuggingFace \\
- Fine-tune the model using the Ceder group's dataset 
-  evaluation of the model. 
- We have three kinds of models: LHS2RHS, RHS2LHS, TGT2CEQ
- Effect of added text (related but not very obviously related) to the generated text. To present the robustness (todo: to include this into the figure)  
- Here, we present many of the abbreviations: left-hand side(LHS), right-hand side (RHS), target compound (TGT), chemical equation(CEQ), and synthesis operation (OPE). 


\begin{figure}[ht!]
\includegraphics[width=\textwidth]{figures/fig_m_tmp.png}
\caption{\textbf{Overview of models for chemical synthesis prediction:}  Prepare data, load a model, fine-tune the model, and evaluate it.
}
\label{fig_overview}
\end{figure}



\subsection*{Data preparation}

-  text-mined database from Ceder group \\
This study utilized a text-mined dataset of inorganic material synthesis recipes (ref: Kononova et al. 2019), which we call the CEDER database. This dataset contains 19,488 synthesis records, automatically extracted from 53,538 paragraphs of scientific literature using natural language processing (NLP) techniques. We extracted balanced chemical reactions, target material, and synthesis operations for each synthesis record in the CEDER database. 

- To generate text using an autoregressive language model, we prepare the training dataset, organized as the pairs of prompt and the target text. The prompt is the text, which works as the seed of the text generation. The target text starts with precisely the same strings as the prompt, followed by the text that we aim to generate. When we load the chemical equations, we connect LHS and RHS by a right arrow, which we write as '$->$.' 


- if we use the synthesis operations (OPE) as the additional prompts, we shrink the synthesis operations in the CEDER dataset to only the sequence of operation names, such as 'Mix Mix Heat Dry,' omitting the details of the experimental condition like the heating temperature, the temperature profile, and the time spent for each operation. 
- the list of operation terms: 'SolutionMix', 'Shape', 'Dry', 'Mix', 'Heat', 'LiquidGrind', 'Quench'

- To make the boundary between the prompt and the generated text clear, we set the separator, which specifies the boundary between the prompt and the answer. 
- Chemical equations in the CEDER database contains short notes about the equations, such that clarification of target compounds and the additives. We removed these notes to make them just the chemical equations organized with LHS and RHS associated with the right arrow.   

\subsection*{Fine-tuning the model}
- Fine-tune the language model: an introduction. 
- we use the distilGPT2 model as the pre-trained model, which can be accessed from HuggingFace. 
- we used the Huggingface API and transformer library to load the model. 
- we referenced distilbert/distilgpt2 to load the model using the class AutoModelForCausalLM.
- We loaded the tokenizer using the AutoTokenizer class. 
- Data collator (DataCollatorForLanguageModeling) and its purpose. 
- We used Trainer to fine-tune the model.
- hyperparameters 
lr=2e-5, 
wdecay=0.01, 
per-device-train-batch-size = 4,  
- We split train and test dataset by ratio 9:1
- cross-validation: 100 epochs, 10-fold cross-validation. We trained the model twice and spent 200 epochs so that the loss function ultimately converges. 
- Supplementary Information covers the training process part. 


\subsection*{Text Inference and Evaluation}
. Text generation: introduction (keyword: autoregressive model).    \\
- We used the fine-tuned model to predict the chemical equation of our target. 
- There are several schemes to generate texts: Greedy Decoding, Contrastive Search, Multinomial Sampling, Beam-Search Decoding, Beam-Search Multinomial Sampling, and Diverse Beam-Search Decoding (we can introduce the schemes briefly, but do not need to spend to go deep). 

% - the chemical equation does need to be the 

% - Option for the text generation (e.g., greedy decoding, multinomial sampling, beam-search decoding). 

- In this work, we apply beam-search multinomial sampling ('num beams':2, 'do sample':True, 'num beam groups':1) . This strategy explores multiple potential sequences simultaneously (beams) and selects the one with the highest overall probability. Here, tokens are sampled according to their probability distribution, introducing randomness and diversity into the generated text.

- Autoregressive text generation model can generate redundant text by repeating the same phrases repeatedly. We can force the generated text to terminate at some specified lengths to avoid too much text. 
- We can guess the lengths of the chemical equation outputs by searching the correlation of the input and output text (e.g. LHS vs RHS). 
- However, this time we want to evaluate the prediction accuracy of the generated text, so we terminate the text by exactly the same lengths as the ground truth equations. Note that deciding the generated text lengths is valid only when we know the ground-truth equation. If we do not know the ground truth, it is necessary to make a guess based on the dataset.  
- SI analyzes the relationship of the text lengths of LHS, RHS, TGT, and CEQ. 

. Evaluation    \\
- evaluation of the predicted text is important in LLM project.     \\
- There exists language evaluation methods such as Levenshtein, cosine similarity, Jaccard, BLEU, ROUGE, ... (we can introduce the schemes briefly, but do not need to spend to go deep) \\
- the use of the evaluation function varies depending on the purpose, like whether we value the correspondence of single characters or close contexts even with different writing expressions.   \\

- When the generated text is a chemical equation, we need a unique evaluation method.  
- what is unique about the chemical equation prediction?    \\
- chemical equations are different from the human conversation language in that they are organized with chemical symbols, numerical symbols, and some special symbols.  
- both LHS and RHS are organized with several chemical formulas connected with '+' symbols     \\
- To regard the predicted chemical equations as correct, we need to have the sequences of chemical elements match the ground truth but accept the permutation of chemical species within the composition.    \\
- for example, we can identify that 'NaCl' and 'ClNa' as the same compounds, thus we should give zero as the penalty of the prediction.     \\
- we can also accept the permutation of the chemical formulas within a set of formulas.  \\
- for example, 'HCl + NaOH' and 'NaOH + HCl' should be identified as the same equations.  \\
- On the other hand, when we evaluate the accuracy of full chemical equation prediction, we need to make sure LHS and RHS do not mix, meaning composition in LHS should not show up in RHS.  \\
- We split the chemical equation with $->$, and evaluate LHS and RHS separately. We then take the average of LHS and RHS as the accuracy of the total equations.   \\

The Tanimoto similarity\cite{bajusz2015tanimoto, holliday2003analysis, godden2000combinatorial} is widely used to evaluate the similarity between two chemical compositions based on their elemental compositions. Given two chemical formulas, the similarity can be computed by treating each formula as a vector in the space of elemental counts. We expanded this Tanimoto similarity to compare the similarity of the two chemical equations so that we can respect the permutation of the composition's orders, which we call the TANI score. 

Let us define the two chemical formulas $comp_1$ and $comp_2$. These formulas can be represented as vectors $\mathbf{v}_1$ and $\mathbf{v}_2$, where each component corresponds to the count of a particular element in the composition.

First, we represent the elemental composition of a formula by a vector of element counts. For each chemical formula, we extract the elements and their respective counts and represent the formula as a vector:

\begin{equation}
\mathbf{v}_1 = \{ \text{element}_1: c_{11}, \text{element}_2: c_{12}, \dots \}
\end{equation}
\begin{equation}
\mathbf{v}_2 = \{ \text{element}_1: c_{21}, \text{element}_2: c_{22}, \dots \}
\end{equation}

where $c_{ij}$ is the count of element $i$ in composition $j$. The similarity is calculated by first determining the common elements between the two vectors, $\mathbf{v}_1$ and $\mathbf{v}_2$, denoted by the set of common elements $E_{\text{common}}$. The dot product between these two vectors is calculated as:

\begin{equation}
\mathbf{v}_1 \cdot \mathbf{v}_2 = \sum_{\text{element} \in E_{\text{common}}} c_{1,\text{element}} \times c_{2,\text{element}}
\end{equation}

Next, we compute the sum of squares of the counts in both vectors:

\begin{equation}
| \mathbf{v}_1 |^2 = \sum_{\text{element} \in \mathbf{v}_1} c_{1,\text{element}}^2
\end{equation}
\begin{equation}
| \mathbf{v}_2 |^2 = \sum_{\text{element} \in \mathbf{v}_2} c_{2,\text{element}}^2
\end{equation}

Finally, the Tanimoto similarity $T(\mathbf{v}_1, \mathbf{v}_2)$ is defined as:

\begin{equation}
T(\mathbf{v}_1, \mathbf{v}_2) = \frac{\mathbf{v}_1 \cdot \mathbf{v}_2}{| \mathbf{v}_1 |^2 + | \mathbf{v}_2 |^2 - \mathbf{v}_1 \cdot \mathbf{v}_2}
\end{equation}

This formula ensures that the similarity ranges from 0 (no similarity) to 1 (identical compositions). If the two compositions share no common elements, the similarity is zero. Otherwise, the value reflects the proportional overlap in their elemental compositions.

We implement this approach by first converting each chemical formula into a vector of element counts and applying the Tanimoto similarity formula to return the similarity score based on the necessary dot product and the sum of squares.

In the context of chemical equations, evaluating the similarity between two equations requires splitting them into their constituent chemical formulas, specifically the reactants and products. We first parse the reactants and products for each equation by splitting the equation at the reaction arrow (commonly represented as "$\rightarrow$"). The formulas in each part are further broken down into individual components (i.e., chemical formulas), which are used for comparison.

Here we define two chemical equations, $eq_1$ and $eq_2$, where each equation contains a set of reactants and products. Denote the set of reactants and products for each equation as $\mathbf{R}_1$, $\mathbf{P}_1$, $\mathbf{R}_2$, and $\mathbf{P}_2$. To compare these equations, we first split them into their respective reactants and products:

\begin{equation}
eq_1: \mathbf{R}_1 \rightarrow \mathbf{P}_1
\end{equation}
\begin{equation}
eq_2: \mathbf{R}_2 \rightarrow \mathbf{P}_2
\end{equation}

Once the equations are split into reactants and products, we compare each component using the Tanimoto similarity. For each pair of formulas in the reactant sets $\mathbf{R}_1$ and $\mathbf{R}_2$, we compute their similarity based on their elemental compositions. The Tanimoto similarity gives the similarity for each pair of formulas, $\mathbf{v}_1$ and $\mathbf{v}_2$. Computing the similarities for all composition pairs, we construct the similarity matrix ($\mathbf{V}\in \mathcal{R}^{N_\text{1} \times N_\text{2}}$). Here, $V_{ij}$-element represents the similarity score of i-th formula in ground-truth equation $\mathbf{R}_1$ (total $N_\text{2}$ terms) and j-th formula of the predicted equation $\mathbf{R}_2$ (total $N_\text{2}$ terms). Linear sum assignment list up the pairs of compositions with the highest similarity. We average the similarity of these corresponding compositions and regard it as the prediction accuracy of two sets o formulas $\mathbf{R}_1$ and $\mathbf{R}_2$. The same process is applied to compare the product sets, $\mathbf{P}_1$ and $\mathbf{P}_2$.

We average the Tanimoto coefficients across the bijective mapping between ground truth compounds and predicted compounds, resulting in naively a “similarity score” as a performance metric. To account for the similarity of the entire equation, the overall similarity is computed as the average of the reactants and products similarities:

\begin{equation}
\text{similarity}_{\text{overall}} = \frac{T(\mathbf{R}_1, \mathbf{R}_2) + T(\mathbf{P}_1, \mathbf{P}_2)}{2}
\end{equation}

In addition to the Tanimoto similarity, the Jaccard similarity is employed as a benchmarking metric. The Jaccard similarity measures the similarity between two sets by comparing their intersection and union. For two sets of formulas (e.g., reactants or products), the Jaccard similarity is given by:

\begin{equation}
J(A, B) = \frac{|A \cap B|}{|A \cup B|}
\end{equation}

$A$ and $B$ represent the sets of elements in the respective formulas. The Jaccard similarity (JAC) helps quantify the structural similarity of the chemical equations based on the overlap of their components.  One distinct point of our Tanimoto similarity score is that it accepts the permutation of the atoms within the formula and the naive evaluation of the chemical formula. While Jaccard similarity requires each predicted formula to be the same as the ground truth to give the similarity score. However, our Tanimoto similarity score takes the similarity, even if the two formulas are not exactly the same. This makes our Tanimoto similarity score more flexible to the chemical equation prediction. Also, the original Jaccard similarity score evaluates LHS and RHS together. Therefore, there is a risk that gives a similarity score when the composition of LHS shows up in RHS. 

\begin{figure}[ht!]
\begin{center}
\includegraphics[width=\textwidth]{figures/fig_m_similaritymethod.png}
\caption{Similarity score calculation method}
\label{fig_similaritymethod}
\end{center}
\end{figure}


 




==> archive/result_240918.tex <==
\section{Results and Discussion}


\subsection{Prediction of one side of the chemical equation given another side of the chemical equation.}

We predict one side of the chemical equation and give another side of the equation. 

LHS2RHS: predict RHS given LHS 
LHS2RHS: predict RHS given LHS 

LHS2RHS (Left-Hand Side to Right-Hand Side) allows the chemists to guess what will be synthesized by the starting compounds in the end, enabling them to reduce the trial and error for guessing the reactions. 
On the other hand, RHS2LHS (Right-Hand Side to Left-Hand Side) lets the user guess what kind of compounds we need to prepare so that they can get the specific target compounds and the byproducts. 

LLM learns the relationship between the reactant and the product in the chemical equation. 
To achieve this task, LLM needs to capture. 
- the collection of the elements in the chemical compositions stabilizing the product compounds. 
- Balance the count of the elements between LHS and RHS. 


Figure \ref{fig_lhs_rhs} shows the schematics and the result of LHS2RHS and RHS2LHS. 
Following the nature of the auto-regressive language model, we represent the dataset so that the prompt is followed by the target text to be generated. As we present in Fig. \ref{fig_lhs_rhs}a,  the LHS2RHS uses the reactants of the chemical equation as the prompt and generates the products of the chemical equation as the target text. The separator symbol '$->$' is given just after the LHS prompt, so that the generated RHS can follow it. Fig. \ref{fig_lhs_rhs}b shows that the RHS2LHS gives the products of the chemical equation as the prompt and generates the reactants of the chemical equation. The separator symbol '$<-$' shows the termination of the RHS prompt, followed by the generated LHS text.


Figure \ref{fig_lhs_rhs}c-f plots the average prediction accuracy regarding the atomic number of elements in the chemical equation. We compare the fine-tuned models (blue) with the pre-trained distilGPT2 models before fine-tuning (pink). Figure \ref{fig_lhs_rhs}c,d present the average accuracy plots for LHS2RHS, using the Tanimoto similarity score adapted for equation evaluation and Jaccard similarity, respectively. Figure \ref{fig_lhs_rhs}e,f shows the result of RHS2LHS. For LHS2RHS and RHS2LHS, the average accuracies over all the element species are below 0.4 with our Tanimoto similarity metric without fine-tuning the model with the CEDER dataset. The pre-trained model tend to give a repetition of the words or characters contained in the prompt, and there appeared a similar chemical formula close to the reactant or products, which made the average prediction accuracy nonzero. However, after fine-tuning the models, LHS2RHS and RHS2LHS gained an accuracy score of 0.869 and 0.911, respectively. Note that these accuracy values based on Tanimoto similarity were overall higher than Jaccard similarity. This result shows the capability of our proposed metric to evaluate the similarity of the sets of chemical formulas by accepting the permutation of formulas and elements. At the same time, the Jaccard score reflects only the permutation of the formulas. Jaccard similarity discards the formulas if there is no exact matching in the opponent set of the formulas. On the other hand, the Tanimoto metrics evaluate the closeness of the two chemical formulas and find out the matching of the formula pairs with the highest similarities. 


Table \ref{tab_main_lhs2rhs} and \ref{tab_main_rhs2lhs} present the examples of prediction results of LHS2RHS and RHS2LHS, respectively. 


Overall, RHS2LHS gave higher accuracy than LHS2RHS. 
- Predicting reactants is easier since the diversity of the available compounds as reactants is limited compared to the products, as there is an almost infinite number of possible inorganic crystals in the whole material space. 
- LHS tends to be formed with multiple well-known species, while RHS is a small number of complex crystals and byproducts. 
- We could observe the nature of the GPT-based model that is better at predicting multiple terms of simple formulas, rather than predicting complex compositions. 


Note that the higher error in the predicted chemical equation does not necessarily mean the incorrect prediction. It might mean that the model outputs a chemical equation that is different from the ground truth. 




\begin{figure}[]
\includegraphics[width=\textwidth]{figures/fig_m_lhs_rhs.pdf}
\caption{\textbf{Schematics and average prediction accuracies for LHS2RHS and RHS2LHS}    \\
Text data representation of \textbf{a.} LHS2RHS and \textbf{b.} RHS2LHS. Given the prompt, the models generate RHS and LHS, respectively. The evaluation metrics compute the prediction accuracy given the generated components of the equations and the ground-truth. \textbf{c-e.} The average prediction accuracy regarding the atomic number of elements in the equations. We used Tanimoto similarity and Jaccard similarity as the metrics. We compare the fine-tuned model (blue) and the original pre-trained model (pink) in each plotting window.
}
\label{fig_lhs_rhs}
\end{figure}


\begin{table}[h!]
\begin{center}
\caption{Selected examples of LHS2RHS results}
\label{tab_main_lhs2rhs}
\begin{tabular}{c|p{5cm}|p{6.5cm}|c|c}
    Model & Prompt (LHS) & Output (RHS) & TANI & JAC \\
\Xhline{5\arrayrulewidth}
True & 2 MnO2 + 0.5 Li2CO3 $\rightarrow$ & 1 LiMn2O4 + 0.5 CO2 + 0.25 O2 & 1.0 & 1.0 \\  
\hline
LHS2RHS  & 2 MnO2 + 0.5 Li2CO3 $\rightarrow$ & 1 LiMn2O4 + 0.5 CO2 + 0.25 O2 & 1.0 & 1.0 \\  
\hline
distilGPT2 & 2 MnO2 + 0.5 Li2CO3 $\rightarrow$ & 0.5 Li2CO3 $\rightarrow$ 0.5 Li2CO3 $\rightarrow$ 0.5 Li2CO3 $\rightarrow$ 0.5 & 0.222 & 0.111  \\  
\Xhline{5\arrayrulewidth}
True & 0.25 Na2CO3 + 0.005 MnO + 0.497 Nb2O5 + 0.25 K2CO3 + 0.004 O2 $\rightarrow$ & 1 (Na0.5K0.5)(Nb0.995Mn0.005)O3 + 0.5 CO2 & 1.0 & 1.0 \\  
\hline
LHS2RHS & 0.25 Na2CO3 + 0.005 MnO + 0.497 Nb2O5 + 0.25 K2CO3 + 0.004 O2 $\rightarrow$ & 1 (K0.5Na0.5)(Nb0.995Mn0.005O3) + 0.5 CO2 & 1.0 & 0.667 \\  
\hline
distilGPT2 & 0.25 Na2CO3 + 0.005 MnO + 0.497 Nb2O5 + 0.25 K2CO3 + 0.004 O2 $\rightarrow$ & 0.001 & 0.0 & 0.0 \\  
\Xhline{5\arrayrulewidth}
True & 3 TiO2 + 0.5 Fe2O3 + 1.5 La2O3 + 1 Bi2O3 $\rightarrow$ & 1 Bi2La3Ti3FeO15 & 1.0 & 1.0 \\  
\hline
LHS2RHS & 3 TiO2 + 0.5 Fe2O3 + 1.5 La2O3 + 1 Bi2O3 $\rightarrow$ & 1 Bi3La3Ti3FeO15 & 0.996 & 0.333 \\  
\hline
distilGPT2 & 3 TiO2 + 0.5 Fe2O3 + 1.5 La2O3 + 1 Bi2O3 $\rightarrow$ & 0.5 Fe2O4 + 0.5  & 0.15 & 0.0 \\  
\Xhline{5\arrayrulewidth}

\end{tabular}
\end{center}
\end{table}


\begin{table}[h!]
\begin{center}
\caption{Selected examples of RHS2LHS results}
\label{tab_main_rhs2lhs}
\begin{tabular}{c|p{5cm}|p{6.5cm}|c|c}
    Model & Prompt (RHS) & Output (LHS) & TANI & JAC \\
\Xhline{5\arrayrulewidth}
True &  1 CaCu3Ti4O12 + 1 CO2 $\leftarrow$ & 3 CuO + 4 TiO2 + 1 CaCO3  & 1.0 & 1.0  \\  
\hline
RHS2LHS & 1 CaCu3Ti4O12 + 1 CO2 $\leftarrow$ & 3 CuO + 4 TiO2 + 1 CaCO3 & 1.0 & 1.0 \\  
\hline
dGPT2 & 1 CaCu3Ti4O12 + 1 CO2 $\leftarrow$ & 1 CO2 $\leftarrow$ 1 CO2 $\leftarrow$ 1 CO2 $<$ & 0.259 & 0.1 \\  
\Xhline{5\arrayrulewidth}
True & 1 LiMn2O4 + 1.5 H2O + 0.25 O2 $\leftarrow$ & 1 LiOH·H2O + 2 $\beta$-MnO2  & 1.0 & 1.0  \\  
\hline
RHS2LHS & 1 LiMn2O4 + 1.5 H2O + 0.25 O2 $\leftarrow$ & 1 LiOH·H2O + 2 MnO2 x & 1.0 & 0.571 \\  
\hline
distilGPT2 & 1 LiMn2O4 + 1.5 H2O + 0.25 O2 $\leftarrow$ & 1.5 O2 $\leftarrow$ 1.5 O2 $\leftarrow$ 1. & 0.4 & 0.0 \\  
\Xhline{5\arrayrulewidth}
True &  1 TbBaMn2O6 + 3 CO2 $\leftarrow$ & 1 BaCO3 + 2 MnCO3 + 0.25 Tb4O7 + 0.625 O2  & 1.0 & 1.0 \\
\hline
RHS2LHS &  1 TbBaMn2O6 + 3 CO2 $\leftarrow$ & 1 Mn2O3 + 1 BaCO3 + 0.25 Tb4O7 + 0.125 O2  & 0.962 & 0.545 \\
\hline
distilGPT2 &  1 TbBaMn2O6 + 3 CO2 $\leftarrow$ & TbBaMn2O6 + 3 CO2 $\leftarrow$ TbBaMn2O6 + 3 CO2 $\leftarrow$  & 0.548 & 0.077 \\
\Xhline{5\arrayrulewidth}
\end{tabular}
\end{center}
\end{table}




\subsection{Prediction of full chemical equation given the target compound}

We have shown that LLM has the potential to capture the chemical relationship of the reactant and the products and can give the equation that balances LHS and RHS based on chemical intuition.   
We expand the model for the advanced search: predicting the whole chemical equation given only the target compounds.    
When chemists have an idea of a new crystal, one of the primary discussions is how to discuss how to synthesize it. 
TGT2CEQ (Target to Chemical Equation) model offers a way to predict both LHS and RHS altogether, providing chemists with an idea of what to prepare as the reactants and products, including the byproducts, leading to the correct setup of the crystal synthesis experiments. 


Figure \ref{fig_tgt2ceq} shows the schematics of TGT2CEQ and the resulting plot. As Figure \ref{fig_tgt2ceq}a explains, we give the target compounds as the text generation prompt. Target compound is followed by the separator symbol '$||$', as the termination of the prompt, and the starting point of the text generation. We aim the model to generate the full chemical equations (CEQ) that are organized with the reactants (LHS) followed by the arrow symbol '$->$' and the products (RHS). We compare the generated chemical equation with the ground truth using the evaluation metrics and compute the prediction accuracies that range between 0 and 1. Note that some cases give multiple target compounds, like (\ce{Na2Eu0.07Y0.93MoPO8}, \ce{Na2Eu0.09Y0.91MoPO8}, \ce{Na2Eu0.2Y0.8MoPO8}, \ce{Na2Eu0.4Y0.6MoPO8}, \ce{Na2Eu0.5Y0.5MoPO8}, \ce{Na2Eu0.55Y0.45MoPO8}, \ce{Na2Eu0.6Y0.4MoPO8}, \ce{Na2EuMoPO8}). In that case, the generated equation should be a generalized one, whose product is written as \ce{Na2Y1-xEux(MoO4)(PO4)}, where 'x' is the variable number as the index of the element.  

Figure \ref{fig_tgt2ceq}b,c shows the result of the prediction accuracy of TGT2CEQ using Tanimoto similarity and Jaccard similarity as the metrics. The average accuracy over all the element species is 0.805 after fine-tuning the model with the CEDER dataset, which has gained intense accuracy from the original pre-trained model's performance with an accuracy of 0.003. Table \ref{tab_main_tgt2ceq} presents three examples of the prediction results with TGTCEQ. 
Note that prediction with pre-trained model (i.e., without fine-tuning) showed almost zero accuracy, which is lower than the case of LHS2RHS or RHS2LHS. This is because the auto-regressive model tends to repeatedly generate the sequence of a subset of the target compounds of the complex compositions or the separator symbols, making the raw outputs far from the format of the chemical equations. 

LHS2RHS and RHS2LHS predict only one side of the chemical equation. On the other hand, TGT2CEQ deal with the prediction of the whole chemical equation. One target inorganic crystal could have multiple pathways for synthesis, so it is natural to have multiple possible answers to the prediction results. Therefore, we do not need to argue that the predicted chemical equation is necessarily wrong, even if its prediction accuracy score is low. Still, the model could shed light on the new pathway for prediction pathway, which has not been reported elsewhere. 


\begin{figure}[]
\includegraphics[width=\textwidth]{figures/fig_m_tgt2ceq.pdf}
\caption{\textbf{Schematics and average prediction accuracies for TGT2CEQ}    \\
\textbf{a.} Text data representation of TGT2CEQ. Given the prompt, the models generate RHS and LHS, respectively. The evaluation metrics compute the prediction accuracy by comparing the generated chemical equation and the ground truth. \textbf{b-c.} The average prediction accuracy regarding the atomic number of elements in the equations. We used Tanimoto similarity and Jaccard similarity as the metrics. We compare the fine-tuned model (blue) and the original pre-trained model (pink) in each plotting window.
}
\label{fig_tgt2ceq}
\end{figure}



\begin{table}[h!]
\begin{center}
\caption{Selected examples of TGT2CEQ}
\label{tab_main_tgt2ceq}
\begin{tabular}{c|p{4cm}|p{8cm}|c|c}
    Model & Prompt (TGT) & Output (CEQ) & TANI & JAC \\
\Xhline{5\arrayrulewidth}
True & CaTi4Cu3O12 $||$ & 3 CuO + 4 TiO2 + 1 CaCO3 $\rightarrow$ 1 CaCu3Ti4O12 + 1 CO2 & 1.0 & 1.0 \\
\hline
TGT2CEQ & CaTi4Cu3O12 $||$ & 3 CuO + 4 TiO2 + 1 CaCO3 $\rightarrow$ 1 CaCu3Ti4O12 + 1 CO2 & 1.0 & 1.0 \\
\hline
distilGPT2 & CaTi4Cu3O12 $||$ & $||$ $||$ $||$ $||$ $||$ $||$ $||$ $||$ $||$ $||$ $||$ $||$ $||$ $||$ $||$ $||$ & 0.0 & 0.0 \\
\Xhline{5\arrayrulewidth}
True & Zr0.54Ti0.46PbO3 $||$ & 1 PbO + 0.46 TiO2 + 0.54 ZrO2 $\rightarrow$ 1 Pb(Zr0.54Ti0.46)O3 & 1.0 & 1.0 \\
\hline
TGT2CEQ & Zr0.54Ti0.46PbO3 $||$ & 1 PbO + 0.46 TiO2 + 0.54 ZrO2 $\rightarrow$ 1 PbZr0.54Ti0.46O3  & 1.0 & 0.8 \\
\hline
distilGPT2 & Zr0.54Ti0.46PbO3 $||$ & 0x0 0x0 0x0 0x0 0x0 0x0 0x0 0x0 0x0 0x0 0x0 0x0 0x0 0 & 0.0 & 0.0 \\
\Xhline{5\arrayrulewidth}
True & Zr20Nb20Ni60 $||$ & 20 Zr + 60 Ni + 20 Nb $\rightarrow$ 1 Ni60Nb20Zr20 & 1.0 & 1.0 \\
\hline
TGT2CEQ & Zr20Nb20Ni60 $||$ & 20 Zr + 60 Ni + 20 Nb $\rightarrow$ 1 Ni60Zr20Nb20 & 1.0 & 0.8 \\
\hline
distilGPT2 & Zr20Nb20Ni60 $||$ & 0 $||$ 0 $||$ 0 $||$ 0 $||$ 0 $||$ 0 $||$ 0 $||$ 0 $||$ & 0.0 & 0.0 \\
\Xhline{5\arrayrulewidth}

\end{tabular}
\end{center}
\end{table}




\subsection{Robustness of the chemical equation prediction against the additional prompts}

So far, we have presented three kinds of fine-tuned models for dealing with chemical equation prediction tasks: LHS2RHS, RHS2LHS, and TGT2CEQ. We saw that each model could carry out tasks predicting the whole or one side of the chemical equation by supplementing the consecutive text from the given prompts. 

As the prediction task becomes more complex, the prompt is expected to get more complex, making it hard to find the essential information for predicting the vital information. In other words, the robustness of the chemical equation in the presence of unimportant information is an important task. 

To present the robustness of the chemical equation prediction, we propose the fine-tuned models called LHSOPE2CEQ (Left-Hand Side and Operations to Right-Hand Side), RHSOPE2CEQ (Right-Hand Side and Operations to Left-Hand Side), and TGTOPE2CEQ (Target and Operations to Chemical Equation), which take in the simplified synthesis operations as the additional prompts, and conduct the same prediction tasks as LHS2RHS, RHS2LHS, and TGT2CEQ, respectively. Figure \ref{fig_ope} presents the difference between the text representations and the comparison of the prediction with or without the additional prompt terms. As Fig. \ref{fig_ope}a-c illustrates, the models with OPE are fine-tuned with the additional prompt generated from the sequence of the synthesis operations. Note that adding operations as the combined text prompt could dilute the highly relevant information for prediction, increasing the risk that the prediction accuracy worsens.  

Figure \ref{fig_lhs_rhs}d compares the average prediction accuracies of the fine-tuned models with or without synthesis operations as the additional prompts. We could see that our model could maintain the accuracy of the chemical equation prediction by less than 0.8\% difference from the model without operation prompts, as you can find the average prediction accuracy for all models in Table \ref{tab_main_all}.


\begin{figure}[]
\includegraphics[width=\textwidth]{figures/fig_m_ope.pdf}
\caption{\textbf{Robustness against added text to prompt}  \\ 
Text data representation of \textbf{a.} LHSOPE2RHS, \textbf{b.} RHSOPE2LHS, and \textbf{c.} TGTOPE2CEQ, which takes the simplified synthesis operations (OPE) as the additional prompts. We present the average prediction accuracy for \textbf{d.} LHSOPE2RHS, \textbf{e.} RHSOPE2LHS, and \textbf{f.} TGTOPE2CEQ. We compare the Tanimoto similarity for each task with or without additional OPE prompts (blue and orange, respectively).
}
\label{fig_ope}
\end{figure}


Table \ref{tab_main_all} shows the average accuracy of the chemical equation prediction. 
- RHS2LHS is easier than LHS2RHS. TGT2CEQ is harder than other two. 
- Even with the addition of the text prompt, the prediction accuracy does not get worse. 
- Tanimoto tends to present a higher accuracy score than Jaccard since it can accept the permutation of the symbols within each chemical formula term. 



\begin{table}[h!]
\begin{center}
\caption{Selected examples of TGT2CEQ}
\label{tab_main_all}
\begin{tabular}{c|cccc}
    Metric & \makecell{Tanimoto \\ (fine-tuned)} & \makecell{Jaccard \\ (fine-tuned)} & \makecell{Tanimoto \\ (no fine-tuning)} & \makecell{Jaccard \\ (no fine-tuning)}  \\
\hline
    LHS2RHS & 0.869 & 0.703 & 0.370 & 0.092   \\ 
    RHS2LHS & 0.911 & 0.825 & 0.250 & 0.064   \\
    TGT2CEQ & 0.805 & 0.705 & 0.003 & 0.001  \\
    LHSOPE2RHS & 0.876 & 0.710 & 0.012 & 0.003   \\
    RHSOPE2LHS & 0.908 & 0.824 & 0.082 & 0.032   \\
    TGTOPE2CEQ & 0.802 & 0.705 & 0.001 & 0.002   \\
\end{tabular}
\end{center}
\end{table}









==> archive/si_tab_lhs2rh_241004_01.tex <==
\begin{longtable}{c|c|p{10cm}|c|c}
\caption{Selected examples of LHS2RHS}\label{tab_s_lhs2rhs}\\
No. &  Model & Text & GTS & JS \\
\Xhline{5\arrayrulewidth}
\endfirsthead
\multicolumn{4}{c}%
{{\tablename\ \thetable{} -- continued from previous page}} \\
No. &  Model & Text & GTS & JS \\
\hline
\endhead
\hline
\multicolumn{4}{r}{{Continued on next page}} \\
\endfoot
\hline
\endlastfoot
1 & True & 0.5 TiO2 + 0.66 SrCO3 + 0.25 Nb2O5 + 0.09 Li2CO3 $\rightarrow$ 1 Li0.18Sr0.66Ti0.5Nb0.5O3 + 0.75 CO2 & 1.0 & 1.0 \\
\hline
1 & LHS2RHS & 0.5 TiO2 + 0.66 SrCO3 + 0.25 Nb2O5 + 0.09 Li2CO3 $\rightarrow$  \textcolor{blue}{1 Li0.18Sr0.66Ti0.5Nb0.5O3 + 0.75 CO2} & 1.0 & 1.0 \\
\hline
1 & distilGPT2 & 0.5 TiO2 + 0.66 SrCO3 + 0.25 Nb2O5 + 0.09 Li2CO3 $\rightarrow$ \textcolor{blue}{0.09 Li2CO3 $\rightarrow$ 0.09 Li2CO3 $\rightarrow$ 0.09 Li} & 0.389 & 0.0 \\
\Xhline{5\arrayrulewidth}
2 & True & 0.204 CuO + 0.98 Fe2O3 + 0.153 NiO + 0.663 ZnO $\rightarrow$ 1 (Ni0.15Cu0.2Zn0.65O)1.02(Fe2O3)0.98 & 1.0 & 1.0 \\
\hline
2 & LHS2RHS & 0.204 CuO + 0.98 Fe2O3 + 0.153 NiO + 0.663 ZnO $\rightarrow$  \textcolor{blue}{1 (Ni0.15Cu0.2Zn0.65O)1.02(Fe2O3)0.98} & 1.0 & 1.0 \\
\hline
2 & distilGPT2 & 0.204 CuO + 0.98 Fe2O3 + 0.153 NiO + 0.663 ZnO $\rightarrow$ \textcolor{blue}{0.99 Fe2O3 + 0.09 Fe2O4 + 0.09 Fe2O5 } & 0.321 & 0.0 \\
\Xhline{5\arrayrulewidth}
3 & True & 3 CuO + 4 TiO2 + 1 CaCO3 $\rightarrow$ 1 CaCu3Ti4O12 + 1 CO2 & 1.0 & 1.0 \\
\hline
3 & LHS2RHS & 3 CuO + 4 TiO2 + 1 CaCO3 $\rightarrow$  \textcolor{blue}{1 CaCu3Ti4O12 + 1 CO2} & 1.0 & 1.0 \\
\hline
3 & distilGPT2 & 3 CuO + 4 TiO2 + 1 CaCO3 $\rightarrow$ \textcolor{blue}{1 CaCO3 $\rightarrow$ 1 CaCO3 $\rightarrow$} & 0.389 & 0.167 \\
\Xhline{5\arrayrulewidth}
4 & True & 2 MnO2 + 0.5 Li2CO3 $\rightarrow$ 1 LiMn2O4 + 0.5 CO2 + 0.25 O2 & 1.0 & 1.0 \\
\hline
4 & LHS2RHS & 2 MnO2 + 0.5 Li2CO3 $\rightarrow$  \textcolor{blue}{1 LiMn2O4 + 0.5 CO2 + 0.25 O2} & 1.0 & 1.0 \\
\hline
4 & distilGPT2 & 2 MnO2 + 0.5 Li2CO3 $\rightarrow$ \textcolor{blue}{MnO2 + 0.5 Li2CO3 $\rightarrow$ MnO2 + 0} & 0.477 & 0.182 \\
\Xhline{5\arrayrulewidth}
5 & True & 1 TiO2 + 1 BaCO3 $\rightarrow$ 1 BaTiO3 + 1 CO2 & 1.0 & 1.0 \\
\hline
5 & LHS2RHS & 1 TiO2 + 1 BaCO3 $\rightarrow$  \textcolor{blue}{1 BaTiO3 + 1 CO2} & 1.0 & 1.0 \\
\hline
5 & distilGPT2 & 1 TiO2 + 1 BaCO3 $\rightarrow$ \textcolor{blue}{TiO2 + 1 BaCO3 -} & 0.778 & 0.286 \\
\Xhline{5\arrayrulewidth}
6 & True & 0.5$*$x Gd2O3 + 0.5 Nb2O5 + 0.5-0.5$*$x Bi2O3 $\rightarrow$ 1 Bi1-xGdxNbO4 & 1.0 & 1.0 \\
\hline
6 & LHS2RHS & 0.5$*$x Gd2O3 + 0.5 Nb2O5 + 0.5-0.5$*$x Bi2O3 $\rightarrow$  \textcolor{blue}{1 Bi1-xGdxNbO4} & 1.0 & 1.0 \\
\hline
6 & distilGPT2 & 0.5$*$x Gd2O3 + 0.5 Nb2O5 + 0.5-0.5$*$x Bi2O3 $\rightarrow$ \textcolor{blue}{Gd2O3 $\rightarrow$ Gd2O3} & 0.6 & 0.0 \\
\Xhline{5\arrayrulewidth}
7 & True & 1 SiO2 + 3 SrCO3 $\rightarrow$ 1 Sr3SiO5 + 3 CO2 & 1.0 & 1.0 \\
\hline
7 & LHS2RHS & 1 SiO2 + 3 SrCO3 $\rightarrow$  \textcolor{blue}{1 Sr3SiO5 + 3 CO2} & 1.0 & 1.0 \\
\hline
7 & distilGPT2 & 1 SiO2 + 3 SrCO3 $\rightarrow$ \textcolor{blue}{SiO2 + 3 SrCO3 $\rightarrow$} & 0.655 & 0.25 \\
\Xhline{5\arrayrulewidth}
8 & True & 1 Al2O3 + 1 Ba(NO3)2 $\rightarrow$ 1 BaAl2O4 + 2 NO2 + 0.5 O2  & 1.0 & 1.0 \\
\hline
8 & LHS2RHS & 1 Al2O3 + 1 Ba(NO3)2 $\rightarrow$  \textcolor{blue}{1 BaAl2O4 + 2 NO2 + 0.5 O2 } & 1.0 & 1.0 \\
\hline
8 & distilGPT2 & 1 Al2O3 + 1 Ba(NO3)2 $\rightarrow$ \textcolor{blue}{1 Ba(NO4)2 $\rightarrow$ 1 Ba(NO5)2 $\rightarrow$} & 0.259 & 0.1 \\
\Xhline{5\arrayrulewidth}
9 & True & 1 SiO2 + 2 CaCO3 $\rightarrow$ 1 Ca2SiO4 + 2 CO2  & 1.0 & 1.0 \\
\hline
9 & LHS2RHS & 1 SiO2 + 2 CaCO3 $\rightarrow$  \textcolor{blue}{1 Ca2SiO4 + 2 CO2 } & 1.0 & 1.0 \\
\hline
9 & distilGPT2 & 1 SiO2 + 2 CaCO3 $\rightarrow$ \textcolor{blue}{SiO2 + 2 CaCO3 $\rightarrow$ } & 0.722 & 0.25 \\
\Xhline{5\arrayrulewidth}
10 & True & 1 FeC2O4·2H2O + 1 LiH2PO4 + 0.5 O2 $\rightarrow$ 1 LiFePO4 + 2 CO2 + 3 H2O & 1.0 & 1.0 \\
\hline
10 & LHS2RHS & 1 FeC2O4·2H2O + 1 LiH2PO4 + 0.5 O2 $\rightarrow$  \textcolor{blue}{1 LiFePO4 + 2 CO2 + 3 H2O} & 1.0 & 1.0 \\
\hline
10 & distilGPT2 & 1 FeC2O4·2H2O + 1 LiH2PO4 + 0.5 O2 $\rightarrow$ \textcolor{blue}{1 LiH2PO4 + 0.5 O2 $\rightarrow$ 1 L} & 0.483 & 0.167 \\
\Xhline{5\arrayrulewidth}
11 & True & 40 SiO2 + 20 TiO2 + 40 BaCO3 $\rightarrow$ 1 40BaO-20TiO2-40SiO2 + 40 CO2 & 1.0 & 1.0 \\
\hline
11 & LHS2RHS & 40 SiO2 + 20 TiO2 + 40 BaCO3 $\rightarrow$  \textcolor{blue}{1 40BaO-20TiO2-40SiO2 + 40 CO2} & 1.0 & 1.0 \\
\hline
11 & distilGPT2 & 40 SiO2 + 20 TiO2 + 40 BaCO3 $\rightarrow$ \textcolor{blue}{20 TiO2 + 40 BaCO3 $\rightarrow$ 20 TiO2 } & 0.714 & 0.222 \\
\Xhline{5\arrayrulewidth}
12 & True & 4 MgCO3 + 1 Nb2O5 $\rightarrow$ 1 Mg4Nb2O9 + 4 CO2 & 1.0 & 1.0 \\
\hline
12 & LHS2RHS & 4 MgCO3 + 1 Nb2O5 $\rightarrow$  \textcolor{blue}{1 Mg4Nb2O9 + 4 CO2} & 1.0 & 1.0 \\
\hline
12 & distilGPT2 & 4 MgCO3 + 1 Nb2O5 $\rightarrow$ \textcolor{blue}{MgCO3 + 1 Nb2O5 $\rightarrow$} & 0.691 & 0.25 \\
\Xhline{5\arrayrulewidth}
13 & True & 0.8+0.2$*$x TiO2 + 0.3$*$x CaCO3 + 1-0.3$*$x BaCO3 + 0.2-0.2$*$x ZrO2 $\rightarrow$ 1 (1-x)Ba(Zr0.2Ti0.8)O3-x(Ba0.7Ca0.3)TiO3 + 1 CO2 & 1.0 & 1.0 \\
\hline
13 & LHS2RHS & 0.8+0.2$*$x TiO2 + 0.3$*$x CaCO3 + 1-0.3$*$x BaCO3 + 0.2-0.2$*$x ZrO2 $\rightarrow$  \textcolor{blue}{1 (1-x)Ba(Zr0.2Ti0.8)O3-x(Ba0.7Ca0.3)TiO3 + 1 CO2} & 1.0 & 1.0 \\
\hline
13 & distilGPT2 & 0.8+0.2$*$x TiO2 + 0.3$*$x CaCO3 + 1-0.3$*$x BaCO3 + 0.2-0.2$*$x ZrO2 $\rightarrow$ \textcolor{blue}{0.3$*$x CaCO3 + 1-0.3$*$x CaCO3 + 1-0.3$*$x CaCO3 + 1-0} & 0.383 & 0.125 \\
\Xhline{5\arrayrulewidth}
14 & True & 1 ZnO + 0.2 Mg(OH)2·4MgCO3·6H2O $\rightarrow$ 1 ZnO-MgO + 0.8 CO2 + 1.4 H2O & 1.0 & 1.0 \\
\hline
14 & LHS2RHS & 1 ZnO + 0.2 Mg(OH)2·4MgCO3·6H2O $\rightarrow$  \textcolor{blue}{1 ZnO-MgO + 0.8 CO2 + 1.4 H2O} & 1.0 & 1.0 \\
\hline
14 & distilGPT2 & 1 ZnO + 0.2 Mg(OH)2·4MgCO3·6H2O $\rightarrow$ \textcolor{blue}{0.2 Mg(OH)2·4MgCO3·6H2O $\rightarrow$ 0.} & 0.238 & 0.0 \\
\Xhline{5\arrayrulewidth}
15 & True & 1 NiO + 0.5 V2O5 + 0.5 Li2CO3 $\rightarrow$ 1 LiNiVO4 + 0.5 CO2 & 1.0 & 1.0 \\
\hline
15 & LHS2RHS & 1 NiO + 0.5 V2O5 + 0.5 Li2CO3 $\rightarrow$  \textcolor{blue}{1 LiNiVO4 + 0.5 CO2} & 1.0 & 1.0 \\
\hline
15 & distilGPT2 & 1 NiO + 0.5 V2O5 + 0.5 Li2CO3 $\rightarrow$ \textcolor{blue}{0.5 Li2CO3 $\rightarrow$ 0.5 L} & 0.35 & 0.125 \\
\Xhline{5\arrayrulewidth}
16 & True & 2 NH4H2PO4 + 1 CaCO3 + 0.5 Y2O3 + 0.5 K2CO3 $\rightarrow$ 1 KCaY(PO4)2 + 1.5 CO2 + 3 H2O + 2 NH3  & 1.0 & 1.0 \\
\hline
16 & LHS2RHS & 2 NH4H2PO4 + 1 CaCO3 + 0.5 Y2O3 + 0.5 K2CO3 $\rightarrow$  \textcolor{blue}{1 KCaY(PO4)2 + 1.5 CO2 + 3 H2O + 2 NH3 } & 1.0 & 1.0 \\
\hline
16 & distilGPT2 & 2 NH4H2PO4 + 1 CaCO3 + 0.5 Y2O3 + 0.5 K2CO3 $\rightarrow$ \textcolor{blue}{0.5 K2CO3 $\rightarrow$ 0.5 K2CO3 $\rightarrow$ 0.5 K2CO3 $\rightarrow$ } & 0.175 & 0.0 \\
\Xhline{5\arrayrulewidth}
17 & True & 1 CaSO4 + 1 KCl $\rightarrow$ 1 KCaSO4Cl & 1.0 & 1.0 \\
\hline
17 & LHS2RHS & 1 CaSO4 + 1 KCl $\rightarrow$  \textcolor{blue}{1 KCaSO4Cl} & 1.0 & 1.0 \\
\hline
17 & distilGPT2 & 1 CaSO4 + 1 KCl $\rightarrow$ \textcolor{blue}{CaSO4 + 1 } & 0.45 & 0.25 \\
\Xhline{5\arrayrulewidth}
18 & True & 1 LiOH·H2O + 2 $\gamma$-MnOOH + 0.25 O2 $\rightarrow$ 1 LiMn2O4 + 2.5 H2O & 1.0 & 1.0 \\
\hline
18 & LHS2RHS & 1 LiOH·H2O + 2 $\gamma$-MnOOH + 0.25 O2 $\rightarrow$  \textcolor{blue}{1 LiMn2O4 + 2.5 H2O} & 1.0 & 1.0 \\
\hline
18 & distilGPT2 & 1 LiOH·H2O + 2 $\gamma$-MnOOH + 0.25 O2 $\rightarrow$ \textcolor{blue}{0.25} & 0.0 & 0.0 \\
\Xhline{5\arrayrulewidth}
19 & True & 1 FeC2O4·2H2O + 1 NH4H2PO4 + 0.5 Li2CO3 + 0.5 O2 $\rightarrow$ 1 LiFePO4 + 2.5 CO2 + 3.5 H2O + 1 NH3 & 1.0 & 1.0 \\
\hline
19 & LHS2RHS & 1 FeC2O4·2H2O + 1 NH4H2PO4 + 0.5 Li2CO3 + 0.5 O2 $\rightarrow$  \textcolor{blue}{1 LiFePO4 + 2.5 CO2 + 3.5 H2O + 1 NH3} & 1.0 & 1.0 \\
\hline
19 & distilGPT2 & 1 FeC2O4·2H2O + 1 NH4H2PO4 + 0.5 Li2CO3 + 0.5 O2 $\rightarrow$ \textcolor{blue}{1 NH4H2PO4 + 0.5 O2 $\rightarrow$ 1 NH4H2PO4 + 0} & 0.282 & 0.154 \\
\Xhline{5\arrayrulewidth}
20 & True & 1 SrCO3 + 1 RuO2 + 0.5 La2O3 + 1 MnO2 $\rightarrow$ 1 SrLaMnRuO6 + 1 CO2 + 0.25 O2 & 1.0 & 1.0 \\
\hline
20 & LHS2RHS & 1 SrCO3 + 1 RuO2 + 0.5 La2O3 + 1 MnO2 $\rightarrow$  \textcolor{blue}{1 SrLaMnRuO6 + 1 CO2 + 0.25 O2} & 1.0 & 1.0 \\
\hline
20 & distilGPT2 & 1 SrCO3 + 1 RuO2 + 0.5 La2O3 + 1 MnO2 $\rightarrow$ \textcolor{blue}{1} & 0.0 & 0.167 \\
\Xhline{5\arrayrulewidth}
21 & True & 1 Li2CuO2 + -1 Li $\rightarrow$ 1 LiCuO2 & 1.0 & 1.0 \\
\hline
21 & LHS2RHS & 1 Li2CuO2 + -1 Li $\rightarrow$  \textcolor{blue}{1 LiCuO2} & 1.0 & 1.0 \\
\hline
21 & distilGPT2 & 1 Li2CuO2 + -1 Li $\rightarrow$ \textcolor{blue}{Li $\rightarrow$ Li} & 0.167 & 0.0 \\
\Xhline{5\arrayrulewidth}
22 & True & 0.5 Fe2O3 + 0.5 La2O3 $\rightarrow$ 1 LaFeO3 & 1.0 & 1.0 \\
\hline
22 & LHS2RHS & 0.5 Fe2O3 + 0.5 La2O3 $\rightarrow$  \textcolor{blue}{1 LaFeO3} & 1.0 & 1.0 \\
\hline
22 & distilGPT2 & 0.5 Fe2O3 + 0.5 La2O3 $\rightarrow$ \textcolor{blue}{0.5 Fe2O} & 0.455 & 0.0 \\
\Xhline{5\arrayrulewidth}
23 & True & 0.4 PbO + 0.97 TiO2 + 0.006 (MgCO3)4·Mg(OH)2·5H2O + 0.6 SrCO3 $\rightarrow$ 1 Pb0.4Sr0.6(Ti0.97Mg0.03)O2.97 + 0.624 CO2 + 0.036 H2O & 1.0 & 1.0 \\
\hline
23 & LHS2RHS & 0.4 PbO + 0.97 TiO2 + 0.006 (MgCO3)4·Mg(OH)2·5H2O + 0.6 SrCO3 $\rightarrow$  \textcolor{blue}{1 Pb0.4Sr0.6(Ti0.97Mg0.03)O2.97 + 0.624 CO2 + 0.036 H2O} & 1.0 & 1.0 \\
\hline
23 & distilGPT2 & 0.4 PbO + 0.97 TiO2 + 0.006 (MgCO3)4·Mg(OH)2·5H2O + 0.6 SrCO3 $\rightarrow$ \textcolor{blue}{0.005 (MgCO3)4·Mg(OH)2·5H2O + 0.6 SrCO3 $\rightarrow$ 0.005 (MgCO3} & 0.488 & 0.077 \\
\Xhline{5\arrayrulewidth}
24 & True & 2 C + 1 Si + 3 Ti $\rightarrow$ 1 Ti3SiC2 & 1.0 & 1.0 \\
\hline
24 & LHS2RHS & 2 C + 1 Si + 3 Ti $\rightarrow$  \textcolor{blue}{1 Ti3SiC2} & 1.0 & 1.0 \\
\hline
24 & distilGPT2 & 2 C + 1 Si + 3 Ti $\rightarrow$ \textcolor{blue}{1 Si + 3 } & 0.036 & 0.2 \\
\Xhline{5\arrayrulewidth}
25 & True & 6 Na2CO3 + 6 TiO2 $\rightarrow$ 1 Na12(TiO3)6 + 6 CO2 & 1.0 & 1.0 \\
\hline
25 & LHS2RHS & 6 Na2CO3 + 6 TiO2 $\rightarrow$  \textcolor{blue}{1 Na12(TiO3)6 + 6 CO2} & 1.0 & 1.0 \\
\hline
25 & distilGPT2 & 6 Na2CO3 + 6 TiO2 $\rightarrow$ \textcolor{blue}{Na2CO3 + 6 TiO2 $\rightarrow$ Na} & 0.408 & 0.222 \\
\Xhline{5\arrayrulewidth}
26 & True & 0.5 La2O3 + 1 Mg(OH)2 + 11 Al(OH)3 $\rightarrow$ 1 LaMgAl11O19 + 17.5 H2O  & 1.0 & 1.0 \\
\hline
26 & LHS2RHS & 0.5 La2O3 + 1 Mg(OH)2 + 11 Al(OH)3 $\rightarrow$  \textcolor{blue}{1 LaMgAl11O19 + 17.5 H2O } & 1.0 & 1.0 \\
\hline
26 & distilGPT2 & 0.5 La2O3 + 1 Mg(OH)2 + 11 Al(OH)3 $\rightarrow$ \textcolor{blue}{1 Mg(OH)3 $\rightarrow$ 1 Mg(OH)3 $\rightarrow$} & 0.3 & 0.143 \\
\Xhline{5\arrayrulewidth}
27 & True & 5 TiO2 + 1 Nb2O5 + 5 Li2CO3 $\rightarrow$ 1 5Li2O-1Nb2O5-5TiO2 + 5 CO2 & 1.0 & 1.0 \\
\hline
27 & LHS2RHS & 5 TiO2 + 1 Nb2O5 + 5 Li2CO3 $\rightarrow$  \textcolor{blue}{1 5Li2O-1Nb2O5-5TiO2 + 5 CO2} & 1.0 & 1.0 \\
\hline
27 & distilGPT2 & 5 TiO2 + 1 Nb2O5 + 5 Li2CO3 $\rightarrow$ \textcolor{blue}{1 Nb2O5 + 5 Li2CO3 $\rightarrow$ 1 Nb2O} & 0.593 & 0.333 \\
\Xhline{5\arrayrulewidth}
28 & True & 1 SiO2 + 0.5 Fe2O3 + 1 Li2CO3 $\rightarrow$ 1 Li2FeSiO4 + 1 CO2 + 0.25 O2 & 1.0 & 1.0 \\
\hline
28 & LHS2RHS & 1 SiO2 + 0.5 Fe2O3 + 1 Li2CO3 $\rightarrow$  \textcolor{blue}{1 Li2FeSiO4 + 1 CO2 + 0.25 O2} & 1.0 & 1.0 \\
\hline
28 & distilGPT2 & 1 SiO2 + 0.5 Fe2O3 + 1 Li2CO3 $\rightarrow$ \textcolor{blue}{SiO3 $\rightarrow$ SiO3 $\rightarrow$ SiO3 $\rightarrow$ SiO3 } & 0.25 & 0.0 \\
\Xhline{5\arrayrulewidth}
29 & True & 1 MoO3 + 1 Cs2CO3 $\rightarrow$ 1 Cs2MoO4 + 1 CO2 & 1.0 & 1.0 \\
\hline
29 & LHS2RHS & 1 MoO3 + 1 Cs2CO3 $\rightarrow$  \textcolor{blue}{1 Cs2MoO4 + 1 CO2} & 1.0 & 1.0 \\
\hline
29 & distilGPT2 & 1 MoO3 + 1 Cs2CO3 $\rightarrow$ \textcolor{blue}{Cs2CO3 $\rightarrow$ Cs2CO3 } & 0.421 & 0.0 \\
\Xhline{5\arrayrulewidth}
30 & True & 7 NH4H2PO4 + 10 CaCO3 + 0.5 K2CO3 $\rightarrow$ 1 Ca10K(PO4)7 + 10.5 CO2 + 10.5 H2O + 7 NH3 & 1.0 & 1.0 \\
\hline
30 & LHS2RHS & 7 NH4H2PO4 + 10 CaCO3 + 0.5 K2CO3 $\rightarrow$  \textcolor{blue}{1 Ca10K(PO4)7 + 10.5 CO2 + 10.5 H2O + 7 NH3} & 1.0 & 1.0 \\
\hline
30 & distilGPT2 & 7 NH4H2PO4 + 10 CaCO3 + 0.5 K2CO3 $\rightarrow$ \textcolor{blue}{0.5 K2CO3 $\rightarrow$ 0.5 K2CO3 $\rightarrow$ 0.5 K2CO3 $\rightarrow$ 0.5 } & 0.146 & 0.0 \\
\Xhline{5\arrayrulewidth}
\end{longtable}

